Optimizing Spot Instance Reliability and Security Using Cloud-Native Data and Tools

This paper represents "Cloudlab", a comprehensive, cloud - native laboratory designed to support network security research and training. Built on Google Cloud and adhering to GitOps methodologies, Cloudlab facilitates the the creation, testing, and deployment of secure, containerized workloads using Kubernetes and serverless architectures. The lab integrates tools like Palo Alto Networks firewalls, Bridgecrew for "Security as Code," and automated GitHub workflows to establish a robust Continuous Integration/Continuous Machine Learning pipeline. By providing an adaptive and scalable environment, Cloudlab supports advanced security concepts such as role-based access control, Policy as Code, and container security. This initiative enables data scientists and engineers to explore cutting-edge practices in a dynamic cloud-native ecosystem, fostering innovation and improving operational resilience in modern IT infrastructures.

==> frontmatter/abstract.tex <==
\begin{abstract}
\input{abstract}
\vspace{1in}
\begin{center}\textbf{Summary}\end{center}
\input{summary}
\end{abstract}


==> frontmatter/cover.tex <==
\title{Length-enhanced superlative verbiage}
\author{Franklin Diaz}
\vspace{0.5in}\\
Professional Services\\
Palo Alto Networks
\vspace{1in}}


==> frontmatter/title.tex <==
\title{\mytitle}
\author[1,2]{Franklin E. Diaz\\ }
%\texttt\href{emailto: fdiaz@paloaltonetworks.com}{fdiaz@paloaltonetworks.com}}
%\affil[1]{Palo Alto Networks}
%\affil[2]{Professional Services - Automation}
\begin{titlepage}
	\date{December 27, 2022}
	\maketitle
	%\thispagestyle{empty} % remove page number from title page? 
	\begin{abstract}
		\raggedright
		The goal of this document is to detail the major components of the ``Cloudlab'' network security lab in
		\href{https://cloud.google.com/}{Google Cloud}. The reasoning behind including certain components and design elements is explained. 
		The relationship between security and the lab are detailed to highlight purpose. Security learning objectives are realized
		at every step of the process in the creation and use of this lab. The result is a widely scoped and highly flexible security
		learning environment for data scientists and engineers with focus on development, test, operations, and continuous pipelines.\\
		\vspace{4cm}
		\centering{\href{https://github.com/devsecfranklin/paper-cloud-lab/blob/main/cloudlab.pdf}{ Click here to download latest version.}}

	\end{abstract}
\end{titlepage}

\begin{comment}
Source files for this paper are available: \url{https://github.com/devsecfranklin/paper-cloud-lab/}
\end{comment}

